Exploratory Gradient Boosting for Reinforcement Learning in Complex Domains

High-dimensional observations and complex real-world dynamics present major challenges in reinforcement learning for both function approximation and exploration. We address both of these challenges with two complementary techniques: First, we develop a gradient-boosting style, non-parametric function approximator for learning on $Q$-function residuals. And second, we propose an exploration strategy inspired by the principles of state abstraction and information acquisition under uncertainty. We demonstrate the empirical effectiveness of these techniques, first, as a preliminary check, on two standard tasks (Blackjack and $n$-Chain), and then on two much larger and more realistic tasks with high-dimensional observation spaces. Specifically, we introduce two benchmarks built within the game Minecraft where the observations are pixel arrays of the agent's visual field. A combination of our two algorithmic techniques performs competitively on the standard reinforcement-learning tasks while consistently and substantially outperforming baselines on the two tasks with high-dimensional observation spaces. The new function approximator, exploration strategy, and evaluation benchmarks are each of independent interest in the pursuit of reinforcement-learning methods that scale to real-world domains.

==> background.tex <==
\section{Background}
\label{sec:background}

We consider the standard discounted, model-free reinforcement-learning
setting in which an agent interacts with an environment with the goal of
accumulating high reward. At each time step $t$, the
agent observes its state $s_t$, which might be represented by a
high-dimensional vector, such as the raw visual input
in Figure~\ref{fig:vis_hill}).
The agent then selects an action $a_t$ that modifies
the state of the environment, typically by moving the agent.
Finally, the agent receives some real-valued reward $r_t$.
This process repeats indefinitely.
The agent's goal is to maximize its long-term
discounted reward, 
%\begin{align*}
$
\sum_{t=1}^{\infty} \gamma^{t-1} r_t
$,
%\end{align*}
where $\gamma \in (0,1)$ is a pre-specified discount factor.

For proving theoretical results, this process is typically assumed to
define a Markov decision process (MDP), meaning that (1)~the next state reached
$s_{t+1}$ is a fixed stochastic function that depends only on the
previous state $s_t$ and the action $a_t$ that was executed; and
(2)~that the reward $r_t$ similarly depends only on $s_t$ and $a_t$.

For simplicity, we assume in our development that the
states are in fact fully observable.
However, in many realistic settings, what the agent observes might not
fully define the underlying state; in other words, the environment
might only be a partially observable MDP.
Nevertheless, in practice, it may often be reasonable to use
observations in place of the unobserved state, especially when the
observations are rich and informative.
Alternatively for this purpose, we could use a recent past window of
observations and actions, or even the entire past history.


